The Antenna Base Plays a Crucial Role in Mosquito Courtship Behavior

Mosquitoes are vectors of diseases like malaria, dengue fever, yellow fever, chikungunya and Zika. For mosquito control it is crucial to understand their hearing system, as mosquitoes' courting behavior is mostly auditory. Many nonlinear characteristics of the mosquito hearing organ have been observed through behavioral studies and neural measurements. These enable mosquitoes to detect and synchronize to other mosquitoes. Many hypotheses concerning the role of the flagellum and the fibrillae of the antenna in mosquito hearing have been made, and neural processes have been considered as the origin of the nonlinearities. In this study we introduce a geometric model based on the morphology of the mosquito antenna base. The model produces many of the observed nonlinear characteristics, providing evidence that the base of the antenna plays a crucial role in mosquito hearing. Even without neural processing, the antenna response to sound produces behaviorally relevant cues that can inform about the presence, location and sex of other mosquitoes.

==> contributiontothefield.tex <==
Mosquitoes hear with their antennas. Hearing mediates their courtship behavior. Controlling their courtship behavior is important in the fight against vector-borne diseases, like malaria, dengue fever, yellow fever, chikungunya and Zika. This manuscript presents and evaluates a mathematical model of the mosquito antenna base. Behavioral and neural studies have shown nonlinearities in mosquitoes’ hearing system. These nonlinearities mediate their courtship behavior, as they enable mosquitoes to detect the presence and location of other mosquitoes, and to synchronize with each other to initiate mating. The nonlinearities have mostly been attributed to auditory efferents and not to the antenna itself. Antennas have rather been considered as linear filters. Our model is inspired by the actual shape of the mosquito antenna base. This shape transforms deflection into rotation. Stimulating the model with artificial signals and mosquito recordings produces many of the said nonlinearities. We argue that the transform from deflection to rotation in the antenna base is responsible for many of the observed nonlinearities inside the mosquito hearing system. Consequently, the antenna base plays a crucial role in mosquito hearing, and needs to be considered in order to understand and, eventually, control mosquito courtship behavior.
